CURTAINs for your Sliding Window: Constructing Unobserved Regions by Transforming Adjacent Intervals

We propose a new model independent technique for constructing background data templates for use in searches for new physics processes at the LHC. This method, called CURTAINs, uses invertible neural networks to parametrise the distribution of side band data as a function of the resonant observable. The network learns a transformation to map any data point from its value of the resonant observable to another chosen value. Using CURTAINs, a template for the background data in the signal window is constructed by mapping the data from the side-bands into the signal region. We perform anomaly detection using the CURTAINs background template to enhance the sensitivity to new physics in a bump hunt. We demonstrate its performance in a sliding window search across a wide range of mass values. Using the LHC Olympics dataset, we demonstrate that CURTAINs matches the performance of other leading approaches which aim to improve the sensitivity of bump hunts, can be trained on a much smaller range of the invariant mass, and is fully data driven.

==> tex/figures.tex <==
%%%% FIGURE 1
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/Fig1.pdf}
    \caption{A schematic overview of the \CURTAINs model. 
    A feature $x$ is correlated with $m$, as can be seen from the 2D contour plots for each side-band in blue.
    Samples $\{x_i^1\}_{i=1}^n$ and $\{x_i^2\}_{i=1}^n$ of batch size $n$ are drawn randomly from the two side-bands. 
    % The masses of the pairs, $\{(m_{low}^i, m_{hi}^i)\}_{i=1}^n$, are passed through a function $f$ forming a set of values $\{f\left(m^i_{low},m^i_{hi}\right)\}_{i=1}^n$.
    In the forward pass the samples from \SBone, $\{{x_1}\}_{i=1}^n$, are passed through the conditional INN where each sample $x_1^i$ is conditioned on $f\left(m^i_{low},m^i_{hi}\right)$, producing the set ${\{z_2^i}\}_{i=1}^n$. The cost function is defined as the distance between this output and the sample from \SBtwo $\{{x_2^i}\}_{i=1}^n$.
    In the inverse pass the roles of each side-band are exchanged. In applying the model, any value for $m$ can be chosen as long as the correct inverse or forward pass is applied.
    }
    \label{fig:curtains_model}
\end{figure}

%%%% FIGURE 2
\begin{figure}[h]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/Fig2.pdf}
    \caption{Schematic showing the relative locations of the two side-bands (\SBone and \SBtwo), the signal region (SR) and the two outer-bands (\OBone and \OBtwo) on the resonant observable $m_{JJ}$. In this example, the non-resonant background is shown as a falling blue line, and the signal region is centred at 3.5~TeV, corresponding to the mass of the injected signal, shown not to scale in red.}
    \label{fig:windows}
\end{figure}

%%%% FIGURE 3
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig3}
    \caption{Input, target and transformed data distributions for the base variable set with the addition of $\Delta R_{JJ}$, for transforming data from \SBone to \SBtwo (left) and \SBtwo to \SBone (right), with the model trained on \SBone (3200~$\leq m_{JJ} <$~3400~GeV) and \SBtwo (3600$~\leq m_{JJ} <$~3800~GeV). The data from \SBone (\SBtwo) is transformed with a forward (inverse) pass of the \CURTAINs model into the target region.
    The diagonal elements show the individual features with the off diagonal elements showing a contour plot between the two observables for the transformed and trained data.}
    \label{fig:curtains_nosignal_SBs}
\end{figure}

%%%% FIGURE 4
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig4}
    \caption{Input, target and transformed data distributions for the base variable set with the addition of $\Delta R_{JJ}$, for transforming data from \SBone to \OBone (left) and \SBtwo to \OBtwo (right), with the model trained on \SBone (3200~$\leq m_{JJ} <$~3400~GeV) and \SBtwo (3600$~\leq m_{JJ} <$~3800~GeV), with \OBone and \OBtwo defined as 200~GeV wide windows directly next to \SBone and \SBtwo away from the signal region.
    The data from \SBone (\SBtwo) is transformed with an inverse (forward) pass of the \CURTAINs model into the target region.
    The diagonal elements show the individual features with the off diagonal elements showing a contour plot between the two observables for the transformed and trained data.}
    \label{fig:curtains_nosignal_OBs}
\end{figure}

%%%% FIGURE 5
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.66\textwidth]{figures/Fig5.pdf}
    \caption{Input, target and transformed data distributions for the base variable set with the addition of $\Delta R_{JJ}$, for transforming data from \SBone and \SBtwo to the signal region to create the background template, with the model trained on \SBone (3200~$\leq m_{JJ} <$~3400~GeV) and \SBtwo (3600$~\leq m_{JJ} <$~3800~GeV). The data from \SBone (\SBtwo) is transformed with a forward (inverse) pass of the \CURTAINs model into the target region.
    The diagonal elements show the individual features with the off diagonal elements showing a contour plot between the two observables for the transformed and trained data.}
    \label{fig:curtains_nosignal_SR}
\end{figure}

%%%% TABLE 1
\begin{table}[htpb]
    \caption {Quantitative agreement between the data distributions of the transformed data and the target data as measured by the AUC of the ROC curve trained on the two samples, as measured for various levels of signal doping with a 200 GeV wide signal region.}
    \label{tab:curtains_aucs}
    \centering
    \begin{tabular}{r c c c c | c}
        \hline
        \hline
        % & \multicolumn{5}{c}{AUC scores}\\
        % \cline{1-6}
        & \SBone\!\!$\rightarrow$\SBtwo & \SBtwo\!$\rightarrow$\SBone & \SBone\!\!$\rightarrow$\OBone & \SBtwo\!$\rightarrow$\OBtwo &  \thead{\SBone\!\!$\rightarrow$SR \\ $\cup$\\ \SBtwo\!$\rightarrow$ SR}\\
        \hline
        
        0 signal    & 0.504 & 0.504 & 0.519 & 0.512 & 0.509   \\
        500 signal  & 0.503 & 0.503 & 0.518 & 0.506 & 0.506   \\
        667 signal  & 0.505 & 0.504 & 0.516 & 0.514 & 0.505   \\
        1000 signal & 0.499 & 0.502 & 0.520 & 0.502 & 0.512   \\
        8000 signal & 0.508 & 0.511 & 0.523 & 0.521 & 0.522   \\
        \hline\hline
    \end{tabular}
\end{table}

%%%% FIGURE 6
\begin{figure}[htpb]
    \centering 
    \includegraphics[width=\textwidth]{figures/Fig6.pdf}
    \caption{Background rejection as a function of signal efficiency (left) and signal improvement as a function of background rejection (right) for the different background template models ($\CURTAINs$ - red, $\CATHODE$ - blue, idealised - green) and a fully supervised classifier (black).
    The sample with 3000 injected signal events in used to train all classifiers in the signal region 3300~$\leq m_{JJ} <$~3700~GeV.
    The solid lines show the mean value of fifty classifier trainings with different random seeds. The uncertainty encompasses 68\% of the runs either side of the mean. 
    }
    \label{fig:ROCandSIC}
\end{figure} 

%%%% FIGURE 7
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/Fig7.pdf}
    \caption{The significance improvement as a function of decreasing signal purity (raw signal events)  for the different background template models ($\CURTAINs$ - red, $\CATHODE$ - blue, idealised - green) and a fully supervised classifier (black). All classifiers trained in the signal region 3300~$\leq m_{JJ} <$~3700~GeV for varying levels of signal doping.
    The solid lines show the mean value of fifty classifier trainings with different random seeds. The uncertainty encompasses 68\% of the runs either side of the mean.}
    \label{fig:dopinglevelscan}
\end{figure}

%%%% FIGURE 8
\begin{figure}[htpb]
    \centering 
    \includegraphics[width=\textwidth]{figures/Fig8}
    \caption{Background rejection as a function of signal efficiency (left) and signal improvement as a function of background rejection (right) for the \CURTAINs (red) and \CATHODE (blue) background template models. The dashed \CATHODE (full) model is trained using all data outside of the signal region, whereas the two solid lines are trained using the default 200~GeV side-bands.
    All classifiers are trained on the sample with 3000 injected signal events for the signal region 3300~$\leq m_{JJ} <$~3700~GeV.
    The lines show the mean value of fifty classifier trainings with different random seeds. The uncertainty encompasses 68\% of the runs either side of the mean. 
    }
    \label{fig:ROCandSIC_cathfull}
\end{figure}

%%%% FIGURE 9
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/Fig9.pdf}
    \caption{The dijet invariant mass for the range of signal regions probed in the sliding window, from 3300~GeV to 4600~GeV, for the case of zero doping.
    Each signal region is 200~GeV wide and split into two 100~GeV wide bins.
    The dashed line shows the expected background after applying a cut on the trained classifier using the \CURTAINs (red) and \CATHODE (blue) methods to produce the background template. Three different cut levels are applied retaining 20\%, 5\% and 0.1\% of background events respectively. The cut values are calculated per signal region using the background template.}
    \label{fig:bumphuntzero}
\end{figure}

%%%% FIGURE 10
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig10.pdf}
    \caption{The dijet invariant mass for the range of signal regions probed in the sliding window, from 3300~GeV to 4600~GeV, for the case of samples doped with 500 (top left), 667 (top right), 1000 (bottom left) and 8000 (bottom right) signal events.
    Each signal region is 200~GeV wide and split into two 100~GeV wide bins .
    The dashed line shows the expected background after applying a cut on the trained classifier using \CURTAINs to produce the background template. Three different cut levels are applied retaining 20\%, 5\% and 0.1\% of background events respectively. The cut values are calculated per signal region using the background template.}
    \label{fig:bumphuntsignal}
\end{figure}
